Sails and Anchors: The Complementarity of Exploratory and Exploitative Scientists in Knowledge Creation

This paper investigates the relationship between scientists' cognitive profile and their ability to generate innovative ideas and gain scientific recognition. We propose a novel author-level metric based on the semantic representation of researchers' past publications to measure cognitive diversity both at individual and team levels. Using PubMed Knowledge Graph (PKG), we analyze the impact of cognitive diversity on novelty, as measured by combinatorial novelty indicators and peer labels on Faculty Opinion. We assessed scientific impact through citations and disruption indicators. We show that the presence of exploratory individuals (i.e., cognitively diverse) is beneficial in generating distant knowledge combinations, but only when balanced by a significant proportion of exploitative individuals (i.e., cognitively specialized). Furthermore, teams with a high proportion of exploitative profiles tend to consolidate science, whereas those with a significant share of both profiles tend to disrupt it. Cognitive diversity between team members appears to be always beneficial to combining more distant knowledge. However, to maximize the relevance of these distant combinations of knowledge, maintaining a limited number of exploratory individuals is essential, as exploitative individuals must question and debate their novel perspectives. These specialized individuals are the most qualified to extract the full potential of novel ideas and integrate them within the existing scientific paradigm.

==> media/table_jebo/nov_f1000.tex <==
\begin{table}[h!]\footnotesize \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.3pt}
\caption{} 
\label{nov_f1000} 
    \scalebox{0.9}{
	\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lccccc| c} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
& \multicolumn{5}{c}{\textit{Dependent variable:}} &  \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{} & \\ 
\\[-1.8ex] & New Finding & Interesting Hyp. &  Technical Adv. & Confirmation & Controversial & \# Obs. \\ 
\hline \\[-1.8ex] 
uzzi\_ref\_fw & -0.118 & -0.037 & 0.365$^{***}$ & -0.380$^{***}$ & -0.288$^{**}$ & 22,934 \\                                             
  & (0.089) & (0.066) & (0.097) & (0.062) & (0.119) & \\  
  & & & & & & \\                                     
 \hline \\[-1.8ex]                                               
 uzzi\_mesh\_fw & -0.392$^{***}$ & 0.115 & 0.342$^{***}$ & -0.229$^{**}$ & -0.239 & 7,896\\                                              
  & (0.101) & (0.099) & (0.117) & (0.117) & (0.184) & \\ 
  & & & & & & \\                                 
 \hline \\[-1.8ex]                                           
 lee\_ref\_fw & 0.169$^{**}$ & 0.060 & 0.077 & -0.478$^{***}$ & -0.277$^{**}$ & 23,941\\                                             
  & (0.084) & (0.065) & (0.094) & (0.072) & (0.137) & \\     
  & & & & & & \\                                      
 \hline \\[-1.8ex]                                               
 lee\_mesh\_fw & -0.338$^{***}$ & 0.025 & 0.444$^{***}$ & -0.272$^{***}$ & -0.114 & 23,949 \\                                             
  & (0.069) & (0.069) & (0.080) & (0.063) & (0.116) & \\         
  & & & & & & \\                                                
 \hline \\[-1.8ex]                                                               
 foster\_ref\_fw & 0.009 & 0.047 & -0.053 & -0.340$^{***}$ & 0.078 & 23,941\\   
  & (0.078) & (0.066) & (0.100) & (0.076) & (0.117) & \\           
  & & & & & & \\                
 \hline \\[-1.8ex]                
 foster\_mesh\_fw & -0.384$^{***}$ & 0.186$^{***}$ & 0.298$^{***}$ & -0.133$^{**}$ & 0.005 &23,949 \\                          
  & (0.078) & (0.060) & (0.075) & (0.067) & (0.137) & \\             
  & & & & & & \\                 
 \hline \\[-1.8ex]               
 wang\_ref\_fw & -0.108$^{**}$ & 0.058 & 0.251$^{***}$ & -0.135$^{***}$ & -0.043 & 23,941\\                               
  & (0.043) & (0.055) & (0.049) & (0.048) & (0.091) & \\    
  & & & & & & \\                 
 \hline \\[-1.8ex]                        
 wang\_mesh\_fw & -0.059 & 0.002 & 0.403$^{***}$ & -0.166$^{***}$ & -0.142$^{*}$ & 23,949\\                                              
  & (0.053) & (0.043) & (0.055) & (0.051) & (0.076) & \\      
  & & & & & & \\                           
 \hline \\[-1.8ex]                                     
shibayama\_abstract\_fw & 0.055 & -0.117$^{*}$ & 0.069 & -0.352$^{***}$ & -0.730$^{***}$ & 23,950 \\                 
  & (0.080) & (0.063) & (0.102) & (0.073) & (0.128) & \\   
  & & & & & & \\                 
 \hline \\[-1.8ex]                                                
 shibayama\_title\_fw & -0.003 & -0.008 & 0.487$^{***}$ & -0.537$^{***}$ & -0.663$^{***}$ & 23,966\\                               
  & (0.081) & (0.067) & (0.090) & (0.057) & (0.118) & \\    
  & & & & & & \\                
 \hline \\[-1.8ex]   
 \hline \\[-1.8ex] 
 \multicolumn{4}{l}{\textit{Note:  Cluster robust SE at journal level \footnote{
 Controls: \# ref, \# mesh, \# aut, year, SJR, journal cat. }}} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
 \end{tabular} 
 \end{threeparttable}
 }
 \end{table} 


==> media/table_jebo/nov_f1000_poisson.tex <==
\begin{table}[h!]\footnotesize \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.3pt}
\caption{} 
\label{nov_f1000_poisson} 
    \scalebox{0.9}{
	\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lccccc| c} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
& \multicolumn{5}{c}{\textit{Dependent variable:}} & \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{} & \\ 
\\[-1.8ex] & New Finding & Interesting Hyp. &  Technical Adv. & Confirmation & Controversial & \# Obs. \\ 
\hline \\[-1.8ex] 
 uzzi\_ref\_fw & -0.107$^{***}$ & -0.073 & 0.269$^{***}$ & -0.341$^{***}$ & -0.340$^{***}$ &  22,934\\
  & (0.025) & (0.057) & (0.082) & (0.056) & (0.112) &\\                                         
 &  & & & & & \\                                                                                
 \hline \\[-1.8ex]     
 uzzi\_mesh\_fw & -0.175$^{***}$ & 0.053 & 0.209$^{**}$ & -0.223$^{**}$ & -0.268 &  7,896\\
  & (0.045) & (0.079) & (0.085) & (0.094) & (0.193) & \\                                
 &  & & & & & \\                                                                       
 \hline \\[-1.8ex]      
 lee\_ref\_fw & -0.064$^{**}$ & -0.008 & 0.029 & -0.414$^{***}$ & -0.325$^{***}$ &  23,941\\
  & (0.026) & (0.055) & (0.072) & (0.062) & (0.126) & \\                                 
 &  & & & & & \\                                                                        
 \hline \\[-1.8ex]                                                                      
 lee\_mesh\_fw & -0.140$^{***}$ & -0.008 & 0.307$^{***}$ & -0.281$^{***}$ & -0.145 &  23,949\\
  & (0.027) & (0.056) & (0.060) & (0.059) & (0.122) & \\                                   
 &  & & & & & \\                                                                          
 \hline \\[-1.8ex]    
 foster\_ref\_fw & -0.090$^{***}$ & -0.006 & -0.111 & -0.288$^{***}$ & 0.040 &  23,941\\
  & (0.025) & (0.049) & (0.075) & (0.064) & (0.112) \\                               
 &  & & & & & \\                                                                      
 \hline \\[-1.8ex]  
 foster\_mesh\_fw & -0.135$^{***}$ & 0.120$^{**}$ & 0.133$^{**}$ & -0.125$^{**}$ & -0.007 &  23,949\\
  & (0.028) & (0.049) & (0.060) & (0.056) & (0.121) & \\                                        
 &  & & & & & \\                                                                               
 \hline \\[-1.8ex]    
 wang\_ref\_fw & -0.032$^{**}$ & 0.024 & 0.181$^{***}$ & -0.117$^{***}$ & -0.089 &  23,941\\
  & (0.015) & (0.043) & (0.046) & (0.045) & (0.087) & \\                                 
 &  & & & & & \\                                                                        
 \hline \\[-1.8ex]     
 wang\_mesh\_fw & 0.015 & 0.019 & 0.356$^{***}$ & -0.136$^{***}$ & -0.112 &  23,949\\
  & (0.015) & (0.032) & (0.043) & (0.045) & (0.072) \\                            
 &  & & & & & \\                                                                   
 \hline \\[-1.8ex]  
 shibayama\_abstract\_fw & -0.021 & -0.120$^{**}$ & 0.145 & -0.296$^{***}$ & -0.772$^{***}$ &  23,950\\
  & (0.020) & (0.052) & (0.099) & (0.063) & (0.120) \\                                            
 &  & & & & & \\                                                                                   
 \hline \\[-1.8ex]          
 shibayama\_title\_fw & -0.047$^{**}$ & -0.015 & 0.446$^{***}$ & -0.428$^{***}$ & -0.639$^{***}$ &  23,966\\
  & (0.022) & (0.050) & (0.082) & (0.048) & (0.115) & \\                                               
 &  & & & & & \\     
  \hline \\[-1.8ex]   
 \hline \\[-1.8ex] 
 \multicolumn{4}{l}{\textit{Note:  Cluster robust SE at journal level \footnote{
 Controls: \# ref, \# mesh, \# aut, year, SJR, journal cat. }}} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $$^{**}$$p$<$0.05; $$^{***}$$p$<$0.01} \\ 
 \end{tabular} 
 \end{threeparttable}
 }
 \end{table} 


==> media/table_jebo/var_description.tex <==

\begin{table}[htbp!]
\centering
\caption{Variable Description} 
\label{tab:vardesc}
\begingroup\tiny

    \scalebox{0.9}{
	\begin{threeparttable}
\begin{tabular}{@{\extracolsep{-5pt}}lll} 

\midrule
\midrule

Variable & Model & Description \\

\midrule 
\multicolumn{3}{c}{Dependent Variables} \\ 
\midrule 
\midrule 

Novelty Variables & & \\ 
\midrule 

\cite{uzzi2013atypical}    &   &  \\
\cite{lee2015creativity}    &   &  \\
\cite{foster2015tradition}    &   &  \\
\cite{wang2017bias}    &   &  \\
\cite{shibayama2021measuring}    &   &  \\

\midrule 
Scientific Impact Variables & & \\ 
\midrule 

Number of citations    &   &  .\\
Disruption$_1noK$    &   &   Following \cite{bornmann1911disruption} \kev{je sais pas lequel}\\
Depth   &   &  Following \cite{bornmann1911disruption} \kev{je sais pas lequel}\\

\midrule 
\multicolumn{3}{c}{Independent Variables} \\
\midrule 
\midrule 

Cognitive Variables & & \\ 
\midrule 

Team cognitive diversity    &   &  The mean of the Inter-authors semantic distance as defined in section \ref{3} with q = 90 for a given paper\\
Average Exploratory profile   &   &  The mean of the Intra-authors semantic distance as defined in section \ref{3} with q = 90 for a given paper\\
Number of Highly exploratory profile    &   &  .\\
Share of highly exploratory profile    &   &  .\\

\midrule 
Control Variables & & \\ 
\midrule 

Number of authors      &   &  .\\
Authors degree of centrality    &   &  .\\
Number of References      &   &  .\\
Number of Meshterms      &   &  .\\
Scimago journal ranking      &   &  .\\
Scimago journal category      &   &  .\\
Year            &   & .\\

\midrule
\bottomrule
 
\end{tabular}%
\endgroup    
 \end{threeparttable}
 }
\end{table}%

==> media/table_jebo/z_faculty_op.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: mar., avr. 18, 2023 - 23:15:11
% Requires LaTeX packages: dcolumn 
\begin{table}[H] \centering 
\renewcommand{\arraystretch}{0.8}
\setlength{\tabcolsep}{0.3pt}
  \caption{} 
  \label{z_faculty_op} 
\small 
    \scalebox{0.9}{
	\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{novelty perceived} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} & \multicolumn{1}{c}{(5)}\\ 
\hline \\[-1.8ex] 
 author\_inter\_abstract (FW) & 0.266$^{***}$ & 0.673$^{**}$ &  &  &  \\ 
  & (0.085) & (0.269) &  &  &  \\ 
  & & & & & \\ 
 author\_intra\_abstract (FW) & -0.414$^{***}$ & -0.498$^{*}$ &  &  &  \\ 
  & (0.103) & (0.266) &  &  &  \\ 
  & & & & & \\ 
 I(author\_inter\_abstract (FW)$\hat{\mkern6mu}$2) &  & -0.435 &  &  &  \\ 
  &  & (0.273) &  &  &  \\ 
  & & & & & \\ 
 I(author\_intra\_abstract (FW)$\hat{\mkern6mu}$2) &  & 0.091 &  &  &  \\ 
  &  & (0.253) &  &  &  \\ 
  & & & & & \\ 
 share\_diverse &  &  & -0.673$^{***}$ & -0.917$^{***}$ & -1.814$^{***}$ \\ 
  &  &  & (0.215) & (0.330) & (0.613) \\ 
  & & & & & \\ 
 share\_typical &  &  & 0.119$^{**}$ & 0.113$^{**}$ & -0.168 \\ 
  &  &  & (0.054) & (0.054) & (0.167) \\ 
  & & & & & \\ 
 I(share\_diverse \textasteriskcentered  share\_typical) &  &  &  & 0.837 & 1.799$^{**}$ \\ 
  &  &  &  & (0.830) & (0.894) \\ 
  & & & & & \\ 
 I(share\_diverse$\hat{\mkern6mu}$2) &  &  &  &  & 1.568 \\ 
  &  &  &  &  & (1.032) \\ 
  & & & & & \\ 
 I(share\_typical$\hat{\mkern6mu}$2) &  &  &  &  & 0.245$^{*}$ \\ 
  &  &  &  &  & (0.137) \\ 
  & & & & & \\ 
 Control variables & YES & YES & YES & YES & YES \\ 
 &  &  &  &  & \\ 
\hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{23,966} & \multicolumn{1}{c}{23,966} & \multicolumn{1}{c}{25,790} & \multicolumn{1}{c}{25,790} & \multicolumn{1}{c}{25,790} \\ 
Log Likelihood & \multicolumn{1}{c}{-15,146.590} & \multicolumn{1}{c}{-15,144.800} & \multicolumn{1}{c}{-16,335.110} & \multicolumn{1}{c}{-16,334.610} & \multicolumn{1}{c}{-16,332.420} \\ 
Akaike Inf. Crit. & \multicolumn{1}{c}{30,581.180} & \multicolumn{1}{c}{30,581.590} & \multicolumn{1}{c}{32,970.220} & \multicolumn{1}{c}{32,971.220} & \multicolumn{1}{c}{32,970.840} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
 \end{threeparttable}
 }
\end{table} 
